Mitigating Dataset Imbalance via Joint Generation and Classification

Supervised deep learning methods are enjoying enormous success in many practical applications of computer vision and have the potential to revolutionize robotics. However, the marked performance degradation to biases and imbalanced data questions the reliability of these methods. In this work we address these questions from the perspective of dataset imbalance resulting out of severe under-representation of annotated training data for certain classes and its effect on both deep classification and generation methods. We introduce a joint dataset repairment strategy by combining a neural network classifier with Generative Adversarial Networks (GAN) that makes up for the deficit of training examples from the under-representated class by producing additional training examples. We show that the combined training helps to improve the robustness of both the classifier and the GAN against severe class imbalance. We show the effectiveness of our proposed approach on three very different datasets with different degrees of imbalance in them. The code is available at https://github.com/AadSah/ImbalanceCycleGAN .

==> ECCV ArXiv Submission/CAM/gradcam_comparison_cub.tex <==
\begin{table*}[htbp]
\setlength\tabcolsep{2pt}%%
\centering
\begin{tabular}{|c|c|c|c|}
\multicolumn{4}{c}{\textbf{GradCAM} heatmaps for \textbf{CUB} dataset}\\
\hline
Original Image&
Vanilla Mode &
ALT Mode &
AUG Mode\\
\hline

\includegraphics[width=1in, height=1in]{CAM/CUB/Original/Olive_sided_Flycatcher_0027_2569956722.jpg} & 
  \includegraphics[width=1in]{CAM/CUB/Bias/cam_Bias_FC_Olive_sided_Flycatcher_0027_2569956722.jpg}&
 \includegraphics[width=1in]{CAM/CUB/ALT/cam_ALT_FC_Olive_sided_Flycatcher_0027_2569956722.jpg} &
 \includegraphics[width=1in]{CAM/CUB/Aug/cam_Aug_FC_Olive_sided_Flycatcher_0027_2569956722.jpg}\\
 
 \includegraphics[width=1in, height=1in]{CAM/CUB/Original/Least_Flycatcher_0022_2494066424.jpg} & 
  \includegraphics[width=1in]{CAM/CUB/Bias/cam_Bias_FC_Least_Flycatcher_0022_2494066424.jpg}& \includegraphics[width=1in]{CAM/CUB/ALT/cam_ALT_FC_Least_Flycatcher_0022_2494066424.jpg}&
   \includegraphics[width=1in]{CAM/CUB/Aug/cam_Aug_FC_Least_Flycatcher_0022_2494066424.jpg}\\
 
 \includegraphics[width=1in, height=1in]{CAM/CUB/Original/Least_Flycatcher_0016_258180172.jpg} & 
  \includegraphics[width=1in]{CAM/CUB/Bias/cam_Bias_FC_Least_Flycatcher_0016_258180172.jpg}&
  \includegraphics[width=1in]{CAM/CUB/ALT/cam_ALT_FC_Least_Flycatcher_0016_258180172.jpg} &
 \includegraphics[width=1in]{CAM/CUB/Aug/cam_Aug_FC_Least_Flycatcher_0016_258180172.jpg} \\
 
 \includegraphics[width=1in, height=1in]{CAM/CUB/Original/Great_Crested_Flycatcher_0032_1989175128.jpg} & 
\includegraphics[width=1in]{CAM/CUB/Bias/cam_Bias_FC_Great_Crested_Flycatcher_0032_1989175128.jpg}&
\includegraphics[width=1in]{CAM/CUB/ALT/cam_ALT_FC_Great_Crested_Flycatcher_0032_1989175128.jpg} &
\includegraphics[width=1in]{CAM/CUB/Aug/cam_Aug_FC_Great_Crested_Flycatcher_0032_1989175128.jpg}\\

\includegraphics[width=1in, height=1in]{CAM/CUB/Original/Great_Crested_Flycatcher_0017_1573235193.jpg} & 
\includegraphics[width=1in]{CAM/CUB/Bias/cam_Bias_FC_Great_Crested_Flycatcher_0017_1573235193.jpg}&
\includegraphics[width=1in]{CAM/CUB/ALT/cam_ALT_FC_Great_Crested_Flycatcher_0017_1573235193.jpg} &
\includegraphics[width=1in]{CAM/CUB/Aug/cam_Aug_FC_Great_Crested_Flycatcher_0017_1573235193.jpg} \\

\hline

\end{tabular}
\caption{\textbf{GradCAM} heatmaps of images from \textbf{CUB} dataset. In each of the rows the leftmost  column (col 1)  shows  the  original image  while  col 2-4 show  GradCAM heatmaps for Vanilla, ALT and AUG Modes respectively (importance increases from blue to red). The column sub-headings denote the corresponding classifier. Note that the heatmaps are generated for the predicted output by the classifiers. Improvement in the explanations can be observed for the ALT and AUG Mode classifiers as compared to the corresponding Vanilla classifier.}
\label{tab:gradcam_CUB}
\end{table*}


==> ECCV ArXiv Submission/CAM/gradcam_comparison_h2z.tex <==
\begin{table*}[htbp]
\setlength\tabcolsep{2pt}%%
\centering
\begin{tabular}{|c|c|c|c|}
\multicolumn{4}{c}{\textbf{GradCAM} heatmaps for \textbf{Horse2Zebra} dataset}\\
\hline
Original Image&
Vanilla Mode &
ALT Mode &
AUG Mode\\
\hline

\includegraphics[width=1in, height=1in]{CAM/H2Z_Cam_images/Original/n02391049_2407.jpg} & 
\includegraphics[width=1in]{CAM/H2Z_Cam_images/Bias/69_cam_Bias_Zebra_n02391049_2407.jpg}&
\includegraphics[width=1in]{CAM/H2Z_Cam_images/ALT/69_cam_ALT_Zebra_n02391049_2407.jpg}&
\includegraphics[width=1in]{CAM/H2Z_Cam_images/Aug/69_cam_Aug_Zebra_n02391049_2407.jpg}  \\

\includegraphics[width=1in, height=1in]{CAM/H2Z_Cam_images/Original/n02391049_2916.jpg} & 
\includegraphics[width=1in]{CAM/H2Z_Cam_images/Bias/101_cam_Bias_Zebra_n02391049_2916.jpg}&
\includegraphics[width=1in]{CAM/H2Z_Cam_images/ALT/101_cam_ALT_Zebra_n02391049_2916.jpg}&
\includegraphics[width=1in]{CAM/H2Z_Cam_images/Aug/101_cam_Aug_Zebra_n02391049_2916.jpg}\\

\includegraphics[width=1in, height=1in]{CAM/H2Z_Cam_images/Original/n02391049_6690.jpg} & 
\includegraphics[width=1in]{CAM/H2Z_Cam_images/Bias/190_cam_Bias_Zebra_n02391049_6690.jpg}&
\includegraphics[width=1in]{CAM/H2Z_Cam_images/ALT/190_cam_ALT_Zebra_n02391049_6690.jpg}&
\includegraphics[width=1in]{CAM/H2Z_Cam_images/Aug/190_cam_Aug_Zebra_n02391049_6690.jpg}  \\
 
\includegraphics[width=1in, height=1in]{CAM/H2Z_Cam_images/Original/n02391049_343.jpg} & 
\includegraphics[width=1in]{CAM/H2Z_Cam_images/Bias/128_cam_Bias_Zebra_n02391049_343.jpg}&
\includegraphics[width=1in]{CAM/H2Z_Cam_images/ALT/128_cam_ALT_Zebra_n02391049_343.jpg}&
\includegraphics[width=1in]{CAM/H2Z_Cam_images/Aug/128_cam_Aug_Zebra_n02391049_343.jpg} \\
 

\includegraphics[width=1in, height=1in]{CAM/H2Z_Cam_images/Original/n02391049_1150.jpg} & 
\includegraphics[width=1in]{CAM/H2Z_Cam_images/Bias/28_cam_Bias_Zebra_n02391049_1150.jpg}&
\includegraphics[width=1in]{CAM/H2Z_Cam_images/ALT/28_cam_ALT_Zebra_n02391049_1150.jpg}&
\includegraphics[width=1in]{CAM/H2Z_Cam_images/Aug/28_cam_Aug_Zebra_n02391049_1150.jpg}  \\


\hline
\end{tabular}
\vspace{2mm}
\caption{\textbf{GradCAM} heatmaps of images from \textbf{Horse2Zebra} dataset. In each of the rows the leftmost  column (col 1)  shows  the  original image  while  col 2-4 show  GradCAM heatmaps for Vanilla, ALT and AUG Modes respectively (importance increases from blue to red). The column sub-headings denote the corresponding classifier. Note that the heatmaps are generated for the predicted output by the classifiers. Improvement in the explanations can be observed for the ALT and AUG Mode classifiers as compared to the corresponding Vanilla classifier.}
\label{tab:gradcam_H2Z}
\end{table*}


==> ECCV ArXiv Submission/GeneratedImages/ALT_images_CUB.tex <==
\begin{table*}[htbp]
\setlength\tabcolsep{2pt}%%
\centering
\begin{tabular}{|c||c|c||c|c|}
\hline
  \textbf{Real}&
\includegraphics[width=1in,height=0.85in]{figs/figsCUB/flycatcher/Baird_Sparrow_0023_3046631067.jpg} &
\includegraphics[width=1in,height=0.85in]{figs/figsCUB/flycatcher/Baird_Sparrow_0023_3046631067.jpg} &
\includegraphics[width=1in,height=0.85in]{figs/figsCUB/sparrow/Acadian_Flycatcher_0012_443003714.jpg} &
\includegraphics[width=1in,height=0.85in]{figs/figsCUB/sparrow/Acadian_Flycatcher_0012_443003714.jpg}
\\
\hline
\hline
% \\
% \vspace{2mm}
 \textbf{$\gamma$}&
\textbf{CycleGAN } &
\textbf{ALT-Mode }&
\textbf{CycleGAN } &
\textbf{ALT-Mode }\\
~ &\textbf{Flycatcher} &
\textbf{Flycatcher }&
\textbf{Sparrow} &
\textbf{Sparrow}\\
\hline
 \textbf{250/12}&
\includegraphics[width=1in,height=0.85in]{figs/figsCUB/flycatcher/00} &
\includegraphics[width=1in,height=0.85in]{figs/figsCUB/flycatcher/01} &
\includegraphics[width=1in,height=0.85in]{figs/figsCUB/sparrow/00.png} &
\includegraphics[width=1in,height=0.85in]{figs/figsCUB/sparrow/01} \\
\hline
 \textbf{250/25}&
\includegraphics[width=1in,height=0.85in]{figs/figsCUB/flycatcher/10} &
\includegraphics[width=1in,height=0.85in]{figs/figsCUB/flycatcher/11} &
\includegraphics[width=1in,height=0.85in]{figs/figsCUB/sparrow/10.png} &
\includegraphics[width=1in,height=0.85in]{figs/figsCUB/sparrow/11} \\
\hline
 \textbf{250/50}&
\includegraphics[width=1in,height=0.85in]{figs/figsCUB/flycatcher/20} &
\includegraphics[width=1in,height=0.85in]{figs/figsCUB/flycatcher/21} &
 \includegraphics[width=1in,height=0.85in]{figs/figsCUB/sparrow/20.png} &
\includegraphics[width=1in,height=0.85in]{figs/figsCUB/sparrow/21} \\
\hline
  \textbf{250/75}&
\includegraphics[width=1in,height=0.85in]{figs/figsCUB/flycatcher/30} &
\includegraphics[width=1in,height=0.85in]{figs/figsCUB/flycatcher/31} &
 \includegraphics[width=1in,height=0.85in]{figs/figsCUB/sparrow/30.png} &
\includegraphics[width=1in,height=0.85in]{figs/figsCUB/sparrow/31} \\
\hline
 \textbf{250/100}&
\includegraphics[width=1in,height=0.85in]{figs/figsCUB/flycatcher/40} &
\includegraphics[width=1in,height=0.85in]{figs/figsCUB/flycatcher/41} &
\includegraphics[width=1in,height=0.85in]{figs/figsCUB/sparrow/40.png} &
\includegraphics[width=1in,height=0.85in]{figs/figsCUB/sparrow/41} \\
\hline
\textbf{250/125}&
\includegraphics[width=1in,height=0.85in]{figs/figsCUB/flycatcher/50} &
\includegraphics[width=1in,height=0.85in]{figs/figsCUB/flycatcher/51} &
\includegraphics[width=1in,height=0.85in]{figs/figsCUB/sparrow/50.png} &
\includegraphics[width=1in,height=0.85in]{figs/figsCUB/sparrow/51} \\
\hline
\end{tabular}
\vspace{2mm}
\caption{Comparison of generated images from only CycleGAN and our ALT Mode trained model for Fine grainedCUB dataset. $\gamma$ indicates the imabalance ratio which is defined as the number of training examples in the majority class to the same in the minority class. Here sparrow is the majority class while flycatcher is the minority class. The top row indicates the input images to the generators of both cycleGAN and ALT mode trained model. Subsequently, every row indicates the generated images from both the models respectively for the imbalance ratio mentioned in leftmost column.}
\label{tab:CUBfig}
\end{table*}


==> ECCV ArXiv Submission/GeneratedImages/ALT_images_H2Z.tex <==
%\begin{figure*}[H]
\begin{table*}[htbp]
\setlength\tabcolsep{2pt}%%
\centering
\begin{tabular}{|c||c|c||c|c|}
\hline
  \textbf{Real}&
 \includegraphics[width=1in]{figs/figsH2Z/zebra/real_horse.jpg} &
 \includegraphics[width=1in]{figs/figsH2Z/zebra/real_horse.jpg} &
 \includegraphics[width=1in]{figs/figsH2Z/horse/real.jpg} &
 \includegraphics[width=1in]{figs/figsH2Z/horse/real.jpg} 
 \\
 \hline
 \hline

% \vspace{2mm}
  \textbf{$\gamma$}&
 \textbf{CycleGAN} &
 \textbf{ALT-Mode } &
 \textbf{CycleGAN } &
 \textbf{ALT-Mode }\\
  ~ &\textbf{Zebra} &
\textbf{Zebra }&
\textbf{Horse} &
\textbf{Horse}\\
 \hline
 \textbf{450/25}&
 \includegraphics[width=1in]{figs/figsH2Z/zebra/00.png} &
 \includegraphics[width=1in]{figs/figsH2Z/zebra/01.png} &
 \includegraphics[width=1in]{figs/figsH2Z/horse/00.png} &
 \includegraphics[width=1in]{figs/figsH2Z/horse/01.png} \\
 \hline
 \textbf{450/50}&
 \includegraphics[width=1in]{figs/figsH2Z/zebra/10.png} &
 \includegraphics[width=1in]{figs/figsH2Z/zebra/11.png} &
 \includegraphics[width=1in]{figs/figsH2Z/horse/10.png} &
 \includegraphics[width=1in]{figs/figsH2Z/horse/11.png} \\
 \hline
 \textbf{450/75}&
 \includegraphics[width=1in]{figs/figsH2Z/zebra/20.png} &
 \includegraphics[width=1in]{figs/figsH2Z/zebra/21.png} &
 \includegraphics[width=1in]{figs/figsH2Z/horse/20.png} &
 \includegraphics[width=1in]{figs/figsH2Z/horse/21.png} \\
 \hline
  \textbf{450/100}&
 \includegraphics[width=1in]{figs/figsH2Z/zebra/30.png} &
 \includegraphics[width=1in]{figs/figsH2Z/zebra/31.png} &
 \includegraphics[width=1in]{figs/figsH2Z/horse/30.png} &
 \includegraphics[width=1in]{figs/figsH2Z/horse/31.png} \\
 \hline
\end{tabular}
\vspace{2mm}
\caption{Comparison of generated images from only CycleGAN and our ALT Mode trained model for Horse2Zebra dataset. $\gamma$ indicates the imabalance ratio which is defined as the number of training examples in the majority class to the same in the minority class. Here horse is the majority class and zebra is the minority class. The top row indicates the input images to the generators of both cycleGAN and ALT mode trained model. Subsequently, every row indicates the generated images from both the models respectively for the imbalance ratio mentioned in the leftmost column.}
\label{tab:horse2zebrafig}
\end{table*}


==> ECCV ArXiv Submission/RISE/rise_comparison_cub.tex <==
\begin{table*}[htbp]
\setlength\tabcolsep{2pt}%%
\centering
\begin{tabular}{|c|c|c|c|}
\multicolumn{4}{c}{\textbf{RISE} heatmaps for \textbf{CUB} dataset}\\
\hline

 Original Image &
 Vanilla Mode &
 ALT Mode &
 AUG Mode\\
 \hline

\includegraphics[width=1in, height=1in]{RISE/CUB/Original/88_CUB_fc_Biased.jpg}&
\includegraphics[width=1in]{RISE/CUB/Bias/88_CUB_fc_Biased.jpg}&
\includegraphics[width=1in]{RISE/CUB/ALT/88_CUB_fc_ALT.jpg} &
\includegraphics[width=1in]{RISE/CUB/Aug/88_CUB_fc_Aug.jpg} \\


\includegraphics[width=1in, height=1in]{RISE/CUB/Original/57_CUB_fc_Biased.jpg}&
\includegraphics[width=1in]{RISE/CUB/Bias/57_CUB_fc_Biased.jpg}&
\includegraphics[width=1in]{RISE/CUB/ALT/57_CUB_fc_ALT.jpg} &
\includegraphics[width=1in]{RISE/CUB/Aug/57_CUB_fc_Aug.jpg} \\

\includegraphics[width=1in, height=1in]{RISE/CUB/Original/55_CUB_fc_Biased.jpg}&
\includegraphics[width=1in]{RISE/CUB/Bias/55_CUB_fc_Biased.jpg}&
\includegraphics[width=1in]{RISE/CUB/ALT/55_CUB_fc_ALT.jpg} &
\includegraphics[width=1in]{RISE/CUB/Aug/55_CUB_fc_Aug.jpg} \\

\includegraphics[width=1in, height=1in]{RISE/CUB/Original/39_CUB_fc_Biased.jpg}&
\includegraphics[width=1in]{RISE/CUB/Bias/39_CUB_fc_Biased.jpg}&
\includegraphics[width=1in]{RISE/CUB/ALT/39_CUB_fc_ALT.jpg} &
\includegraphics[width=1in]{RISE/CUB/Aug/39_CUB_fc_Aug.jpg} \\


\includegraphics[width=1in, height=1in]{RISE/CUB/Original/89_CUB_fc_Biased.jpg}&
\includegraphics[width=1in]{RISE/CUB/Bias/89_CUB_fc_Biased.jpg}&
\includegraphics[width=1in]{RISE/CUB/ALT/89_CUB_fc_ALT.jpg} &
\includegraphics[width=1in]{RISE/CUB/Aug/89_CUB_fc_Aug.jpg} \\

\hline

\end{tabular}

\vspace{2mm}
\caption{\textbf{RISE} heatmaps of images from \textbf{CUB} dataset. In each of the rows the leftmost  column (col 1)  shows  the  original image of the Flycatcher while  col 2-4 show  RISE heatmaps for Vanilla, ALT and AUG Modes respectively (importance increases from blue to red). The column sub-headings denote the corresponding classifier. Note that the heatmaps are generated for the predicted output by the classifiers. Improvement in the explanations can be observed for the ALT and AUG Mode classifiers as compared to the corresponding Vanilla classifier.}
\label{tab:rise_cub}
\end{table*}


==> ECCV ArXiv Submission/RISE/rise_comparison_h2z.tex <==
\begin{table*}[htbp]
\setlength\tabcolsep{2pt}%%
\centering
\begin{tabular}{|c|c|c|c|}
\multicolumn{4}{c}{\textbf{RISE} heatmaps for \textbf{Horse2Zebra} dataset}\\
\hline

 Original Image &
 Vanilla Mode &
 ALT Mode &
 AUG Mode\\
 \hline

\includegraphics[width=1in, height=1in]{RISE/H2Z/original/45_H2Z_zebra_Biased.jpg}&
\includegraphics[width=1in]{RISE/H2Z/Bias/45_H2Z_zebra_Biased.jpg}&
\includegraphics[width=1in]{RISE/H2Z/ALT/45_H2Z_zebra_ALT.jpg} &
\includegraphics[width=1in]{RISE/H2Z/Aug/45_H2Z_zebra_Aug.jpg} \\

\includegraphics[width=1in, height=1in]{RISE/H2Z/original/41_H2Z_zebra_Biased.jpg}&
\includegraphics[width=1in]{RISE/H2Z/Bias/41_H2Z_zebra_Biased.jpg}&
\includegraphics[width=1in]{RISE/H2Z/ALT/41_H2Z_zebra_ALT.jpg} &
\includegraphics[width=1in]{RISE/H2Z/Aug/41_H2Z_zebra_Aug.jpg} \\

\includegraphics[width=1in, height=1in]{RISE/H2Z/original/216_H2Z_zebra_Biased.jpg}&
\includegraphics[width=1in]{RISE/H2Z/Bias/216_H2Z_zebra_Biased.jpg}&
\includegraphics[width=1in]{RISE/H2Z/ALT/216_H2Z_zebra_ALT.jpg} &
\includegraphics[width=1in]{RISE/H2Z/Aug/216_H2Z_zebra_Aug.jpg} \\

\includegraphics[width=1in, height=1in]{RISE/H2Z/original/165_H2Z_zebra_Biased.jpg}&
\includegraphics[width=1in]{RISE/H2Z/Bias/165_H2Z_zebra_Biased.jpg}&
\includegraphics[width=1in]{RISE/H2Z/ALT/165_H2Z_zebra_ALT.jpg} &
\includegraphics[width=1in]{RISE/H2Z/Aug/165_H2Z_zebra_Aug.jpg} \\

\includegraphics[width=1in, height=1in]{RISE/H2Z/original/20_H2Z_zebra_Biased.jpg}&
\includegraphics[width=1in]{RISE/H2Z/Bias/20_H2Z_zebra_Biased.jpg}&
\includegraphics[width=1in]{RISE/H2Z/ALT/20_H2Z_zebra_ALT.jpg} &
\includegraphics[width=1in]{RISE/H2Z/Aug/20_H2Z_zebra_Aug.jpg} \\


\hline


\end{tabular}

\vspace{2mm}
\caption{\textbf{RISE} heatmaps of images from \textbf{Horse2Zebra} dataset. In each of the rows the leftmost  column (col 1)  shows  the  original image of the Zebra while  col 2-4 show  RISE heatmaps for Vanilla, ALT and AUG Modes respectively (importance increases from blue to red). The column sub-headings denote the corresponding classifier. Note that the heatmaps are generated for the predicted output by the classifiers. Improvement in the explanations can be observed for the ALT and AUG Mode classifiers as compared to the corresponding Vanilla classifier.}
\label{tab:rise_h2z}

\end{table*}


==> ECCV ArXiv Submission/results/ACSA_F2S.tex <==
\begin{table*}[htbp]
\setlength\tabcolsep{12pt}
\centering
\resizebox{\textwidth}{!}{ 
\begin{tabular}{l||ccccccccccccc}
\hline
\textbf{Dataset} & \multicolumn{6}{c}{\textbf{CUB-200-2011}}\\
\hline
\#Flycatcher                 & 12     & 25     & 50     & 75     & 100    & 125    \\
\hline
\hline
Vanilla                      & 0.5060 & 0.5320 & 0.5800 & 0.5960 & 0.6660 & 0.6900 \\
\hline
US               & 0.5040 & 0.5980 & 0.6340 & 0.6860 & 0.6880 & 0.6680 \\
TS                 & 0.5060 & 0.5320 & 0.5800 & 0.5980 & 0.6101 & 0.6840 \\
CS              & 0.5800 & 0.6400 & 0.6300 & 0.6800 & 0.7000 & 0.7200 \\
OS                & 0.5140 & 0.5540 & 0.6080 & 0.6420 & 0.6860 & 0.6840 \\
US + CS & 0.5380 & 0.5780 & 0.6520 & 0.6620 & 0.6640 & 0.6960 \\
OS + CS  & 0.5440 & 0.5960 & 0.6500 & 0.6520 & 0.6740 & 0.7040 \\
SMOTE     ~\cite{Chawla2002Smote}                    & 0.5100 & 0.6200 & 0.6460 & 0.6280 & 0.7060 & 0.7020 \\
CBL~\cite{Cui2019Class} ($\beta\!=\!0.9$)                   & 0.5220 & 0.6056 & 0.6460 & 0.6700 & 0.6800 & 0.7180 \\
CBL~\cite{Cui2019Class} ($\beta\!=\!0.99$)                 & 0.5640 & 0.6440 &\textbf{0.6880} & 0.6800 & 0.7000 & 0.6900 \\
CBL~\cite{Cui2019Class} ($\beta\!=\!0.999$)                 & 0.5600 & 0.6460 &0.6760 & 0.6440 & 0.6580 & 0.7220 \\
CBL~\cite{Cui2019Class} ($\beta\!=\!0.9999$)                & 0.5520 & \textbf{0.6640} & 0.6360 & 0.6660 & \textbf{0.7040} & \textbf{0.7280} \\
\hline
ALT Mode                 & 0.5800 & 0.5800 & 0.6280 & 0.6320 & 0.6800 & 0.6160 \\
AUG Mode                  & \textbf{0.6080} & 0.6400 & 0.6620 & \textbf{0.7080} & 0.6980 & 0.7180 \\
\hline                             
\end{tabular}}
\vspace{2mm}
%\bigskip
\caption{Comparison of the proposed method on the CUB-200-2011 dataset using both AUG and ALT mode in terms of \textbf{Average Class Specific Accuracy (ASCA)}. The class specific accuracy is averaged over the two classes (Sparrow and Flycatcher). The number of majority class training images (Sparrow) is fixed to 250. We provide the ACSA for all the imbalance ratios starting from 250:12 (Sparrow:Flycatcher) to 250:125 (Sparrow:Flycatcher) images in the training set. We can see that our proposed approach is better or at par with the other methods.
%\abir{Add the citations. Basically copy from main paper}
}
\label{tab:acsa_cub}
\end{table*}

==> ECCV ArXiv Submission/results/ACSA_H2Z.tex <==
\begin{table}[htbp]
\setlength\tabcolsep{14pt}
\centering
\resizebox{\linewidth}{!}{ 
\begin{tabular}{l||cccc}
\hline
\textbf{Dataset} & \multicolumn{3}{c}{\textbf{Horse2Zebra}}\\
\hline
\#Zebra                       & 25             & 50             & 75            & 100                   \\
\hline
\hline
Vanilla &0.5150 &0.6940 &0.7800 &0.8100 \\
\hline
US                & 0.5000            & 0.8080          & 0.8640         & 0.8640                 \\
TS                 & 0.5090          & 0.7290          & 0.7740         & 0.8290                 \\
CS               & 0.8240          & 0.8533   & 0.8820         & \textbf{0.8787} \\
OS                & 0.65733   & 0.8333   & 0.8580         & 0.87330         \\
US + CS & 0.5133   & 0.7800           & 0.8773 & 0.8820                 \\
OS + CS  & 0.7927   & 0.8667   & 0.8807  & 0.8820                 \\
SMOTE     ~\cite{Chawla2002Smote}                    & 0.5627   & 0.7847   & 0.8260         & 0.8500                  \\
CBL~\cite{Cui2019Class} ($\beta\!=\!0.9$)                 & 0.8067   & 0.8520          & 0.8727  & 0.8640                 \\
CBL~\cite{Cui2019Class} ($\beta\!=\!0.99$)               & 0.8353   & 0.85           & 0.8713 & 0.8740                 \\
CBL~\cite{Cui2019Class} ($\beta\!=\!0.999$)               & 0.8433   & 0.8427   & 0.8673  & 0.8780                 \\
CBL~\cite{Cui2019Class} ($\beta\!=\!0.9999$)              & 0.8380          & 0.8467   & 0.8760         & 0.8773          \\
\hline
ALT Mode                 & 0.8240              & 0.8230          & 0.7980         & 0.8160                 \\
AUG Mode                  & \textbf{0.8670} & \textbf{0.8770} & \textbf{0.8900} & 0.8630                 \\
\hline
\end{tabular}}
\vspace{2mm}
%\bigskip
\caption{Comparison of the proposed method on the Horse2Zebra dataset using both AUG and ALT mode in terms of \textbf{Average Class Specific Accuracy (ASCA)}. The class specific accuracy is averaged over the two classes (Horse and Zebra). The number of majority class training images (Horse) is fixed to 450. We provide the ACSA for all the imbalance ratios starting from 450:25 (Horse:Zebra) to 450:100 (Horse:Zebra) images in the training set. We can see that our proposed approach is comprehensively outperforming the other methods. The ACSA values show that the recall values for both the classes increase on average as a result of the application of imbalance mitigation strategies but our proposed method works best especially in presence of highly skewed training data.
%\abir{Add the citations. Basically copy from main paper}
}
\label{tab:horse2zebra_acsa}
\end{table}

==> ECCV ArXiv Submission/results/ACSA_celebA.tex <==
\begin{table*}[htbp]
\centering
\resizebox{\linewidth}{!}{ 
\begin{tabular}{l||cccccccccc}
\hline
\textbf{Dataset} & \multicolumn{8}{c}{\textbf{CelebA}}\\
\hline
\#Male                       & 50              & 100             & 200             & 300             & 400             & 500             & 600  &700 &800 &900  \\
\hline
\hline
Vanilla &0.5400 &0.6760 &0.8120 &0.86400 &0.9090 &0.9210 &0.9290 &0.9280 &0.9350 &0.9360\\
\hline
US                & 0.8153          & 0.8553          & 0.9040          & \textbf{0.9173} & 0.9187          & \textbf{0.9300} & 0.9220    & 0.9147 & 0.9193 & 0.9223       \\
TS                 & 0.5430          & 0.7290          & 0.8210          & 0.8590          & 0.9030          & 0.9200          & \textbf{0.9300}   & 0.9300 & 0.9350 & 0.9360 \\
CS              & 0.8097          & 0.8250          & 0.9020          & 0.9143          & 0.9253          & 0.9250          & 0.9247         & 0.9277 & 0.9253 & 0.9347  \\
OS                 & 0.7030          & 0.7830          & 0.8823          & 0.9060          & 0.9200          & 0.9193          & 0.9227       & 0.9293 & 0.9320 & 0.9330    \\
US + CS & 0.8003          & 0.8560          & 0.9003          & 0.9143          & 0.9170          & 0.9197          & 0.9247         & 0.9263 & 0.9300 & 0.9230     \\
OS + CS  & 0.8010          & 0.8393          & 0.8947          & 0.9093          & 0.9227          & 0.9260          & 0.9317          & 0.9317 & 0.9300 & \textbf{0.9387} \\
SMOTE  ~\cite{Chawla2002Smote}                       & 0.7197          & 0.8033          & 0.8877          & 0.8940          & 0.9180          & 0.9213          & 0.9290   & 0.9357 &\textbf{0.9383} & 0.9357       \\
CBL~\cite{Cui2019Class} ($\beta\!=\!0.9$)                & 0.7493          & 0.8123          & 0.8917          & 0.9083          & 0.9133          & 0.9213          & 0.9260   &\textbf{ 0.9373} & 0.9283 & 0.9380       \\
CBL~\cite{Cui2019Class} ($\beta\!=\!0.99$)                & 0.7613          & 0.8287          & 0.8980          & 0.9140          & 0.9187          & 0.9237          & 0.9210   & 0.9283 & 0.9343 & 0.9373        \\
CBL~\cite{Cui2019Class} ($\beta\!=\!0.999$)               & 0.7990          & 0.8437          & 0.8980          & 0.9143          & 0.9183          & 0.9237          & 0.9253    & 0.9233 & 0.9327 & 0.9307     \\
CBL~\cite{Cui2019Class} ($\beta\!=\!0.9999$)              & 0.8130          & 0.8320          & 0.9013          & 0.9120          & 0.9240          & 0.9233          & 0.9270   & 0.9313 & 0.9307 & 0.9373       \\
\hline
ALT Mode                 & \textbf{0.8260} & 0.8540          & 0.8880          & 0.8870          & 0.8460          & 0.8930          & 0.8820 &0.8860 &0.8850 &0.8790          \\
AUG Mode                  & 0.8230          & \textbf{0.8800} & \textbf{0.9180} & 0.9160          & \textbf{0.9300} & 0.9210          & 0.9150   &0.9260 &0.9350 &0.9360      \\
\hline
\end{tabular}}
\vspace{2mm}
%\bigskip
\caption{Comparison of the proposed method on the CelebA dataset using both AUG and ALT mode in terms of \textbf{Average Class Specific Accuracy (ASCA)}. The class specific accuracy is averaged over the two classes (Male and Female). The number of majority class training images (Female) in CelebA is fixed to 900. We provide the ACSA for all the imbalance ratios starting from 900:50 (Female:Male) to a perfectly balanced scenario of 900:900 (Female:Male) images in the training set. We can see that our proposed approach is comprehensively outperforming the other methods in the highly imbalanced region (left part of the table) and performing at par with the other methods in the more balanced scenario (towards right of the table). The ACSA values show that the recall values for both the classes increase on average as a result of the application of imbalance mitigation strategies but our proposed method works best especially in presence of highly skewed training data.
%\abir{Add the citations. Basically copy from main paper}
}
\label{tab:celeba_acsa}
\end{table*}

==> ECCV ArXiv Submission/results/f1_female_results.tex <==
\begin{table*}[htbp]
\centering
\resizebox{\linewidth}{!}{ 
\begin{tabular}{l||cccccccccc}
\hline
\textbf{Dataset} & \multicolumn{8}{c}{\textbf{CelebA}}\\
\hline
\#Male                       & 50      & 100     & 200     & 300     & 400     & 500     & 600   &700 &800 &900       \\
\hline
\hline
Vanilla                      & 0.6840  & 0.7560  & 0.8380  & 0.8740  & 0.9120  & 0.9240  & 0.9300  &0.9280 &0.9340 &\textbf{0.9380}       \\
\hline
US                & 0.8261 & 0.8610 & 0.9043 &\textbf{ 0.9170} & 0.9192 & 0.9293 & 0.9217 & 0.9141 & 0.9168 & 0.9210  \\
TS       & 0.6860  & 0.7840  & 0.8440  & 0.8740  & 0.9080  & 0.9220  & 0.9300   & 0.9320  & 0.9340  &\textbf{0.9380}     \\
CS               & 0.8301  & 0.8436  & 0.9060  & 0.9148  & 0.9256  & 0.9255  & 0.9243 & 0.9286  & 0.9250  & 0.9334   \\
OS        & 0.7691  & 0.8170  & 0.8885  & 0.9080  & 0.9218  & 0.9198  & 0.9238      & 0.9301  & 0.9319  & 0.9331        \\
US + CS & 0.7936  & 0.8643  & 0.8986  & 0.9122  & 0.9147  & 0.9172  & 0.9234     & 0.9249  & 0.9277  & 0.9209        \\
OS + CS & 0.8268  & 0.8513  & 0.8973  & 0.9119  & 0.9230  & \textbf{0.9259}  & \textbf{0.9323}     & 0.9320  & 0.9303  & 0.9380          \\
SMOTE  ~\cite{Chawla2002Smote}                       & 0.7774  & 0.8288  & 0.8936  & 0.8981  & 0.9192  & 0.9218  & 0.9294  & 0.9363  &\textbf{0.9379}  & 0.9356     \\
CBL~\cite{Cui2019Class} ($\beta\!=\!0.9$)                 & 0.7963  & 0.8372  & 0.8962  & 0.9104  & 0.9147  & 0.9220  & 0.9260 &\textbf{ 0.9370}  & 0.9284  & 0.9376       \\
CBL~\cite{Cui2019Class} ($\beta\!=\!0.99$)                & 0.8011  & 0.8483  & 0.9017  & 0.9161  & 0.9195  & 0.9247  & 0.9229  & 0.9284  & 0.9338  & 0.9366      \\
CBL~\cite{Cui2019Class} ($\beta\!=\!0.999$)               & 0.8218  & 0.8587  & 0.9031  & 0.9164  & 0.9186  & 0.9252  & 0.9256  &0.9246  & 0.9328  & 0.9296      \\
CBL~\cite{Cui2019Class} ($\beta\!=\!0.9999$)              & 0.8322  & 0.8494  & 0.9047  & 0.9111  & 0.9238  & 0.9240  & 0.9278  & 0.9306  & 0.9306  & 0.9370   \\
\hline
ALT Mode    &0.8300             & 0.8580  & 0.8840  & 0.8820  & 0.8380  & 0.8940  & 0.8820  &0.8820 &0.8860 &0.8780    \\
AUG Mode                 &\textbf{ 0.8360}  & \textbf{0.8820}  & \textbf{0.9160}  & 0.9160  &\textbf{ 0.9300}  & 0.9200  & 0.9160 &0.9260 &0.9320 &0.9320    \\ 
\hline
\end{tabular}}
\vspace{2mm}
%\bigskip
\caption{Comparison of the proposed method on the CelebA dataset using both AUG and ALT mode. The number of majority class training images (female) in CelebA is fixed to 900. Here we provide the \textbf{$F_1$ score of the majority class (Female)} for all the imbalance ratios starting from 900:50 (Female:Male) to a perfectly balanced scenario of 900:900 (Female:Male) images in the training set. We can see that our proposed approach is comprehensively outperforming the other methods in the highly imbalanced region (left part of the table) and performing at par with the other methods in the more balanced scenario (towards right of the table). While Table~\ref{tab:celeba_male_f1} shows that the minority class (male) classification gets improved due to our Cycle-GAN based dataset repairment, it also improves the classification performance of the majority class (female).
%\abir{Remove the demarking line after column 500.}
%\abir{Add the citations. Basically copy from main paper}
}
\label{tab:celebA_female_f1}
\end{table*}

==> ECCV ArXiv Submission/results/f1_horses.tex <==
\begin{table}[htbp]
\setlength\tabcolsep{14pt}
\centering
\resizebox{\linewidth}{!}{ 
\begin{tabular}{l||llll}
\hline
\textbf{Dataset} & \multicolumn{3}{c}{\textbf{Horse2Zebra}}\\
\hline
\#Zebra                      & 25      & 50     & 75     & 100    \\
\hline
\hline
Vanilla                      & 0.6740       & 0.7680       & 0.8200       & 0.8400       \\
\hline
US                & 0.5333       & 0.8217       & 0.8784       & 0.8741       \\
TS                 & 0.6720       & 0.7860       & 0.8160       & 0.8540       \\
CS               & 0.8469       & 0.8692       & 0.8919       & 0.8873       \\
OS                 & 0.7452       & 0.8559       & 0.8742       & 0.8821       \\
US + CS & 0.4410 & 0.8097 & 0.8880 & \textbf{0.8912} \\
OS + CS  & 0.8282       & 0.8779       & 0.8910       & 0.8892       \\
SMOTE ~\cite{Chawla2002Smote}                        & 0.6964       & 0.8205       & 0.8511       & 0.8684       \\
CBL~\cite{Cui2019Class} ($\beta\!=\!0.9$)                 & 0.8373       & 0.8658       & 0.8856       & 0.8790       \\
CBL~\cite{Cui2019Class} ($\beta\!=\!0.99$)                & 0.8537       & 0.8643       & 0.8816       & 0.8856       \\
CBL~\cite{Cui2019Class} ($\beta\!=\!0.999$)               & 0.8569       & 0.8585       & 0.8793       & 0.8862       \\
CBL~\cite{Cui2019Class} ($\beta\!=\!0.999$)             & 0.8560       & 0.8668       & 0.8862       & 0.8868       \\
\hline
ALT Mode                & 0.8380       & 0.8120       & 0.7880       & 0.8120       \\
AUG Mode                  & \textbf{0.8800 }     &\textbf{ 0.8900}      & \textbf{0.8980 }     & 0.8760      \\
\hline
\end{tabular}}
\vspace{2mm}
%\bigskip
\caption{Comparison of the proposed method on the Horse2Zebra dataset using both AUG and ALT mode. The number of majority class training images (Horse) is fixed to 450. Here we provide the \textbf{$F_1$ score of the majority class (Horse)} for all the imbalance ratios starting from 450:25 (Horse:Zebra) to a perfectly balanced scenario of 450:100 (Horse:Zebra) images in the training set. We can see that our proposed approach is comprehensively outperforming the other methods in the highly imbalanced region (left part of the table) and performing at par with the other methods in the more balanced scenario (towards right of the table). While Table 3 in the main paper shows that the minority class (zebra) classification gets improved due to our Cycle-GAN based dataset repairment, it also improves the classification performance of the majority class (horse).
%\abir{Add the citations. Basically copy from main paper}
}
\label{tab:horses_f1}
\end{table}

==> ECCV ArXiv Submission/results/f1_male_results.tex <==
%\documentclass[10pt,twocolumn,letterpaper]{article}
%\begin{document}
\begin{table*}[htbp]
\centering
\resizebox{\linewidth}{!}{ 
\begin{tabular}{l||cccccc||cccccc}
%\multicolumn{12}{c}{\textbf{F1 Score for minority class}} \\
\hline
\textbf{Dataset} & \multicolumn{8}{c}{\textbf{CelebA}}\\
\hline
\#Minority examples              & 50              & 100             & 200             & 300             & 400             & 500  &600 &700 &800 &900  \\
\hhline{=#======#======}
%\hline
Vanilla                      & 0.1500          & 0.5220          & 0.7740          & 0.8460          & 0.9020          & 0.9160  &0.9260 &0.9320 &0.9380 &\textbf{0.9400}        \\
\hline
US                & 0.8029          & 0.8491          & 0.9036          & \textbf{0.9176} & 0.9179          & \textbf{0.9307} & 0.9223 & 0.9152 & 0.9216 & 0.9236 \\
TS                 & 0.1560          & 0.6300          & 0.7880          & 0.8420          & 0.8960          & 0.9200   & 0.9260  &0.9320 &0.9380 &\textbf{0.9400}  \\
CS               & 0.7825          & 0.8012          & 0.8975          & 0.9137          & 0.9250          & 0.9244  & 0.9250 & 0.9267 & 0.9256 & 0.9359   \\

OS                 & 0.5805          & 0.7333          & 0.8749          & 0.9036          & 0.9181          & 0.9188   & 0.9215 & 0.9286 & 0.9321 & 0.9329 \\
US + CS & 0.8041          & 0.8463          & 0.9019          & 0.9163          & 0.9191          & 0.9220  & 0.9259 & 0.9277 & 0.9321 & 0.9250   \\
OS + CS  & 0.7644          & 0.8249          & 0.8916          & 0.9065          & 0.9223          & 0.9260   & 0.9310 & 0.9313 & 0.9297 & 0.9393 \\
SMOTE~\cite{Chawla2002Smote}                        & 0.6208          & 0.7685          & 0.8807          & 0.8895          & 0.9167          & 0.9208 & \textbf{0.9285} & 0.9350 & \textbf{0.9387} & 0.9357 \\
CBL~\cite{Cui2019Class} ($\beta\!=\!0.9$)                 & 0.6736          & 0.7771          & 0.8867          & 0.9061          & 0.9118          & 0.9206   & 0.9260 &\textbf{0.9376} & 0.9282 & 0.9384 \\
CBL~\cite{Cui2019Class} ($\beta\!=\!0.99$)               & 0.7012          & 0.8021          & 0.8938          & 0.9118          & 0.9178          & 0.9226   & 0.9190 & 0.9282 & 0.9348 & 0.9380   \\
CBL~\cite{Cui2019Class} ($\beta\!=\!0.999$)              & 0.7692          & 0.8250          & 0.8922          & 0.9122          & 0.9179          & 0.9220  & 0.9251 & 0.9220 & 0.9326 & 0.9317   \\
CBL~\cite{Cui2019Class} ($\beta\!=\!0.9999$)              & 0.7885          & 0.8099          & 0.8977          & 0.9127          & 0.9241          & 0.9226   & 0.9261 & 0.9320 & 0.9307 & 0.9376  \\
\hline
(ours) ALT Mode              & \textbf{0.8240} & 0.8520          & 0.8900          & 0.8880          & 0.8520          & 0.8920 &0.8860 &0.8880 &0.8840 &0.8760     \\
(ours) AUG Mode               & 0.8060          & \textbf{0.8740} & \textbf{0.9140} & 0.9160 & \textbf{0.9340} & 0.9220   &0.9140  &0.9280 &0.9340 &0.9340 \\
\hline
\end{tabular}}
\vspace{2mm}
%\bigskip
\caption {Comparison of the proposed method on the CelebA dataset using both AUG and ALT mode. The number of majority class training images (female) in CelebA is fixed to 900. Here we provide the \textbf{$F_1$ score of the minority class (Male)} for all the imbalance ratios starting from 900:50 (Female:Male) to a perfectly balanced scenario of 900:900 (Female:Male) images in the training set. The $F_1$ score for imabalance ratio till 900:500 (Female:Male) is replicated from the main paper for completeness.
Our proposed approach outperforms all others comprehensively in the high imbalance regions. The additional ratios show that the traditional methods start to do well as the dataset is more and more balanced. However, our augmented way of training is still very good and the difference in performance is only at the third decimal place in the high 90's.
%\abir{Write the observation here - if 600 onwards gives bad results, tell that we are doing good in the highly imbalanced region which is crucial and tell that our method is very close to the best performing models in balanced scenarios.}
%\abir{Add the citations. Basically copy from main paper}
}
\label{tab:celeba_male_f1}
\end{table*}
%\end{document}

==> ECCV ArXiv Submission/results/f1_male_results_main_paper.tex <==
%\documentclass[10pt,twocolumn,letterpaper]{article}
%\begin{document}
\begin{table*}[t]
\centering
\resizebox{\linewidth}{!}{ 
\begin{tabular}{l||cccccc||cccccc}
%\multicolumn{12}{c}{\textbf{F1 Score for minority class}} \\
\hline
\textbf{Dataset} & \multicolumn{6}{c}{\textbf{CelebA}} & \multicolumn{5}{c}{\textbf{CUB-200-2011}}\\
\hline
\#Minority examples              & 50              & 100             & 200             & 300             & 400             & 500     &12         & 25		  & 50 		& 75  & 100 & 125\\
\hhline{=#======#======}
%\hline
Vanilla                      & 0.1500          & 0.5220          & 0.7740          & 0.8460          & 0.9020          & 0.9160      &0.0240      & 0.1180 		& 0.2960 & 0.3700 & 0.5520 & 0.6160 \\
\hline
TS                 & 0.1560          & 0.6300          & 0.7880          & 0.8420          & 0.8960          & 0.9200   &0.0240 & 0.1180 &0.2880 & 0.3640 & 0.2567 & 0.6080 \\
CS               & 0.7825          & 0.8012          & 0.8975          & 0.9137          & 0.9250          & 0.9244    &0.3674        & 0.5007 		& 0.5001 & 0.6384 & 0.6485 & 0.7212 \\
US                & 0.8029          & 0.8491          & 0.9036          & \textbf{0.9176} & 0.9179          & \textbf{0.9307}  &0.2952 & 0.4263 		& 0.6074 & 0.6893 & \textbf{0.7169} & 0.7080 \\
OS                 & 0.5805          & 0.7333          & 0.8749          & 0.9036          & 0.9181          & 0.9188  &0.0602         & 0.1943 		& 0.3910 & 0.5007 & 0.6295 & 0.6322 \\
US + CS & 0.8041          & 0.8463          & 0.9019          & 0.9163          & 0.9191          & 0.9220    &0.5394       & 0.4760 		& 0.6655 	& 0.6647 & 0.6995 & 0.7201 \\
OS + CS  & 0.7644          & 0.8249          & 0.8916          & 0.9065          & 0.9223          & 0.9260   &0.3845        & 0.4225		& 0.5739 & 0.6147 & 0.6246 & 0.6913 \\
SMOTE~\cite{Chawla2002Smote}                        & 0.6208          & 0.7685          & 0.8807          & 0.8895          & 0.9167          & 0.9208   &0.0586        & 0.4533 		& 0.6375 & 0.5625 & 0.6708 & 0.6674 \\
CBL~\cite{Cui2019Class} ($\beta\!=\!0.9$)                 & 0.6736          & 0.7771          & 0.8867          & 0.9061          & 0.9118          & 0.9206    &0.1342       & 0.4006 		& 0.5068 & 0.5624 & 0.6187 & 0.6890 \\
CBL~\cite{Cui2019Class} ($\beta\!=\!0.99$)               & 0.7012          & 0.8021          & 0.8938          & 0.9118          & 0.9178          & 0.9226      &0.3259     & 0.5392 		& 0.6001 & 0.6196 & 0.6369 & 0.6600 \\
CBL~\cite{Cui2019Class} ($\beta\!=\!0.999$)              & 0.7692          & 0.8250          & 0.8922          & 0.9122          & 0.9179          & 0.9220   &0.3492        & 0.5256 		& 0.6105& 0.5400 & 0.5937 & 0.7212 \\
CBL~\cite{Cui2019Class} ($\beta\!=\!0.9999$)              & 0.7885          & 0.8099          & 0.8977          & 0.9127          & 0.9241          & 0.9226    &0.3562       & 0.5950 		& 0.5138 & 0.5933 &  0.6547 & \textbf{0.7344} \\
\hline
(ours) ALT Mode              & \textbf{0.8240} & 0.8520          & 0.8900          & 0.8880          & 0.8520          & 0.8920     &0.5120        & 0.5120 		& 0.5640 & 0.6340 & 0.6940 &0.5960 \\
(ours) AUG Mode               & 0.8060          & \textbf{0.8740} & \textbf{0.9140} & 0.9160 & \textbf{0.9340} & 0.9220   &\textbf{0.5940}         & \textbf{0.6040} 		& 		\textbf{0.6680} & \textbf{0.7060} & 0.7040 & 0.7180 \\
\hline
\end{tabular}}
\vspace{2mm}
%\bigskip
\caption {Comparison of the proposed method on the CelebA and CUB-200-2011 datasets using both AUG and ALT mode. The left half of the table shows the results for CelebA and the right half shows the results for the pairs of birds chosen from CUB-200-2011 dataset. The number of majority class training images (female) in CelebA is fixed to 900 while the CUB-200-2011 majority class (Sparrow) images 250. Minority class $F_1$ score for both are shown where the individual column headings indicate the number of minority class training images.}
\label{tab:celeba_cub}
\end{table*}
%\end{document}

==> ECCV ArXiv Submission/results/f1_sparrow.tex <==
\begin{table*}[htbp]
\setlength\tabcolsep{12pt}
\centering
\resizebox{1\textwidth}{!}{ 
\begin{tabular}{l||ccccccc}
\hline
\textbf{Dataset} & \multicolumn{6}{c}{\textbf{CUB-200-2011}}\\
\hline
\#Flycatcher                 & 12              & 25                  & 50              & 75              & 100             & 125               \\
\hline
\hline
Vanilla                      & 0.6700          & 0.6800              & 0.7020          & 0.7020          & 0.7340          & 0.7380  \\
\hline
US      & 0.4000         & 0.6694            & 0.6474         & 0.6803         & 0.6470         & 0.6113        \\
TS                 & 0.6720          & 0.6800              & 0.7020          & 0.7060          & 0.6915          & 0.7320    \\
CS      & \textbf{0.6800} & 0.7134              & 0.6994          & 0.7027          & 0.7373          & 0.7184            \\
OS                 & 0.6721          & 0.6916              & 0.7100          & 0.7174          & 0.7261          & 0.7221        \\
US + CS & 0.3058          & 0.6033              & 0.6287    & 0.6573          & 0.6116          & 0.6650       \\
OS + CS  & 0.5712          & 0.6784              & 0.6965          & 0.6808          & 0.7108          & 0.7136       \\
SMOTE  ~\cite{Chawla2002Smote}                       & 0.6685          & 0.6949              & 0.6123          & 0.6478          & 0.7334          & 0.7250        \\
CBL~\cite{Cui2019Class} ($\beta\!=\!0.9$)                & 0.6695          & 0.6028 & 0.7217          & \textbf{0.7317} & 0.7228          & \textbf{0.7381}         \\
CBL~\cite{Cui2019Class} ($\beta\!=\!0.99$)                & 0.6763          & 0.7080              & \textbf{0.7424} & 0.7218          & \textbf{0.7439} & 0.7102           \\
CBL~\cite{Cui2019Class} ($\beta\!=\!0.999$)               & 0.6591          & \textbf{0.7164}     & 0.7149          & 0.7073          & 0.7036          & 0.7210            \\
CBL~\cite{Cui2019Class} ($\beta\!=\!0.999$)              & 0.6523          & 0.7094              & 0.7058          & 0.7142          & 0.7387          & 0.7179              \\
\hline
ALT Mode                 & 0.6260          & 0.6180              & 0.6680          & 0.6160          & 0.6640          & 0.6200      \\
AUG Mode                  & 0.6180         & 0.6660             & 0.6560         & 0.7100         & 0.6900        & 0.7180    \\
\hline
\end{tabular}}
\vspace{2mm}
%\bigskip
\caption{Comparison of the proposed method on the CUB-200-2011 dataset using both AUG and ALT mode. The number of majority class training images (sparrow) is fixed to 250. Here we provide the \textbf{$F_1$ score of the majority class (Sparrow)} for all the imbalance ratios starting from 250:12 (Sparrow:Flycatcher) to 250:125 (Sparrow:Flycatcher) images in the training set. We can see that our proposed approach is not doing good in recovering the $F_1$ score of the majority class in this dataset. This may be due to the presence of very few images for both the classes and also due to the difficult finegrained nature of the task in this particular dataset. The effect can also be seen in Table~\ref{tab:acsa_cub} where the ACSA is just at par for these ratios for the proposed method. However in Table 1 of the main paper we see that the F1 score for the other class (Flycather) is always high for our proposed method.
%\abir{Remove the demarking line after column 500.}
%\abir{Add the citations. Basically copy from main paper}
}
\label{tab:cub_sparrow_f1}
\end{table*}

==> ECCV ArXiv Submission/results/f1_zebra_horse_results.tex <==
\begin{table}[t]
\centering

\resizebox{1.02\linewidth}{!}{  
\begin{tabular}{l||c|c|c|c|c|c|c|c|c|c|c|c||c|c}
\hline
\multirow{2}{*}{\textbf{\#Zebra}} & \multirow{2}{*}{Vanilla} & \multirow{2}{*}{TS} & \multirow{2}{*}{CS} & \multirow{2}{*}{US} & \multirow{2}{*}{OS} & \multirow{2}{*}{US+CS} & \multirow{2}{*}{OS+CS} & \multirow{2}{*}{SMOTE~\cite{Chawla2002Smote}} & \multicolumn{4}{c||}{CBL~\cite{Cui2019Class}} & \multicolumn{2}{c}{Ours}
\\
%\hline
&&&&&&&&& $\beta=0.9$ & $\beta=0.99$ & $\beta=0.999$ & $\beta=0.9999$ & ALT & AUG\\
\hhline{=#=|=|=|=|=|=|=|=|=|=|=|=#=|=}
25& 0.0500 & 0.0340 & 0.7925 & 0.1333 & 0.4750 & 02865 & 0.7366 & 0.2108 & 0.7613 & 0.8116 & 0.8263 & 0.8120 & 0.8040 & \textbf{0.8500}\\
50 & 0.5580 & 0.6260 & 0.8329 & 0.7891 & 0.8012 & 0.7343 & 0.8522 & 0.7298 & 0.8347 & 0.8316 & 0.8222 & 0.8192 & 0.8320 & \textbf{0.8620}\\
75 & 0.7180 & 0.7040 & 0.8699 & 0.8457 & 0.8370 & 0.8644 & 0.8680 & 0.7902 & 0.8562 & 0.8587 & 0.8524 & 0.8633 & 0.8020 & \textbf{0.8780}\\
100 & 0.7680 & 0.7940 & 0.8684 & 0.8521 & 0.8628 & \textbf{0.8711} & 0.8735 & 0.8254 & 0.8446 & 0.8595 & 0.8683 & 0.8657 & 0.8220 & 0.8520\\
\hline
\end{tabular}}
\vspace{0.1mm}
%\bigskip
\caption {\small Performance comparison on Horse2Zebra dataset.
% using both AUG and ALT mode.
The first row lists the approaches against which we have compared our performance.
The number of majority class training images (horses)
% in Horse2Zebra
is fixed at 450 while the number of zebra images used in training is shown as the row headings.
The minority class $F_1$ score is seen to get improved with application of our proposed approach especially in the augmented mode for high imbalance regions.
}
\label{tab:horse2zebra}
\vskip -0.2in
\end{table}

==> ECCV ArXiv Submission/results/gan_performance_results.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}
% \begin{document}
\begin{table*}[t]
\centering
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{c|cc||c|cc||c|cc}                          
\multicolumn{3}{c}{\textbf{Celeb A Dataset}}                      & \multicolumn{3}{c}{\textbf{CUB-200-2011 Dataset}}            & \multicolumn{3}{c}{\textbf{Horse2Zebra Dataset}}          \\
\hline
\# Male & CycleGAN        & ALT Mode & \#Flycatcher & CycleGAN & ALT Mode & \#Zebra & CycleGAN & ALT Mode \\
\hline
50                & \textbf{0.4798} & 0.4677                      & 12                    & 0.4149          & \textbf{0.4554}                            &                         &         &                             \\
100               & 0.5574          & \textbf{0.6220}             & 25                   &  \textbf{0.4238}        &  0.4059                           &  25                       & \textbf{0.3532}         & 0.3480                    \\
200               & 0.7646          & \textbf{0.8152}             & 50                   &  0.4337        &  \textbf{0.4505}                           & 50                        & \textbf{0.3880}         & 0.2680                            \\
300               & 0.7516          & \textbf{0.8200}             &  75                  &  0.4347        &  \textbf{0.4653}                          &75                        & \textbf{0.5000}         & 0.4440                           \\
400               & 0.8122 & \textbf{0.8455}                      &  100                  &  \textbf{0.4317}        &  0.4307                           &  100                       & \textbf{0.5492}         &   0.4780                           \\
500               & 0.8286          & \textbf{0.8457}             &  125                  &  0.4198        & \textbf{0.4604}                            &                         &          &                             \\
                       
\hline
\end{tabular}
\end{adjustbox}
\bigskip
\caption {Comparison of the inception accuracies of the Cycle-GAN before and after applying our proposed dataset repairment approach (in ALT mode). The table is divided into 3 parts from left to right corresponding to the three datasets on which the experimentations are performed. The dataset names are marked as headings of the parts. Each part is further divided into two halves where the left half shows the performance for the vanilla cycle-GAN and the right half shows the same after the cycle-GAN is trained in alternate mode of the proposed approach. The values shown are averaged over 5 runs for each of the cases. For two (CelebA and CUB-200-2011) out of the three datasets, the ALT mode of training improves the Cycle-GAN performance for most of the cases, while for Horse2Zebra dataset the performance is not increasing which may be due to the distintive feature of the dataset where the attributes of the two classes are markedly different.}
\label{tab:gan_perf}
\end{table*}
%\end{document}
